A Night at the LLM Zoo: Data Conditioned Flow Matching for Generating Pretrained LLM Weights

A challenge to Weight Space Learning as it expands from task specific and vision models to Large Language Models (LLMs) is the absence of a well curated and analyzed LLM population. To address this, we train such a model zoo for application to Weight Space Generation by systematically varying the data mixture composition between web text, books, mathematics, coding, and French across populations of 51M, 124M, and 355M parameter GPT-2 Models, each tier with count N = 100. We analyze these populations by cosine similarity, functional diversity, Leave-One-Mixture-Out modeling, and variance decomposition. We show that the zoo contains diverse models whose variation is structured by training mixture composition. We embed the training mixture composition to condition a Flow Matching model of complete pretrained LLM weights in Gram-PCA compressed weight space. By demonstrating zero-shot generalization to held out mixtures, measuring Continuous Ranked Probability Score skill, as well as finding minimal changes in downstream test-set perplexity and general capability benchmark scores, we show that our generator generalizes on the simplex of data mixtures to produce models that perform similarly to those in the zoo ex nihilo. Finally, we produce all source code and artifacts to support the continued expansion of Weight Space Learning and Generation into the LLM domain.

==> fig_plots/generalization.tex <==
\begin{figure}[tbp]
\centering
\includegraphics[width=\textwidth]{figs/generalization.png}
\caption{Advantage over blinded retrieval (a) and the proper score (b) against $L_1$
distance to the nearest mixture seen by the generator. 
Filled markers are equal-count bins over the $80$ \emph{interior} cells with binned 
standard errors. The five vertices are open squares and are excluded from binning.}
\label{fig:generalization}
\end{figure}
